Determinisability of one-clock timed automata

The deterministic membership problem for timed automata asks whether the timed language recognised by a nondeterministic timed automaton can be recognised by a deterministic timed automaton. We show that the problem is decidable when the input automaton is a one-clock nondeterministic timed automaton without epsilon transitions and the number of clocks of the deterministic timed automaton is fixed. We show that the problem in all the other cases is undecidable, i.e., when either 1) the input nondeterministic timed automaton has two clocks or more, or 2) it uses epsilon transitions, or 3) the number of clocks of the output deterministic automaton is not fixed.

==> ex1.tex <==
    \definecolor{accentGray}{RGB}{71, 71, 75}
    \definecolor{accent}{RGB}{252, 199, 18}
    \definecolor{ca}{RGB}{231, 111, 253}
    \definecolor{cb}{RGB}{249, 128, 199}
    \definecolor{cc}{RGB}{254, 157, 101}
    \tikzstyle{letter} = [inner sep=0.8mm, anchor=north west, yshift=-2mm]
    \tikzstyle{bgLine} = [draw=accentGray, line width=0.2mm]
    \tikzstyle{box} = [bgLine, fill=white, inner sep=0.8mm, anchor=north west, outer sep=0, text=black]
    \tikzstyle{dot} = [fill=black, inner sep=0.8mm, outer sep=0]
    \tikzstyle{axis} = [line width=0.5mm, draw=accent, -{Triangle[scale=1]}]

%    \begin{center}
        \begin{tikzpicture}[xscale=1.9,yscale=0.75]
                      % \node at (0,0.8) {};
                      % \node at (0,-0.8) {};
            \node[text width=1.5cm, anchor=east, align=right] at (7.5,0.0) {\footnotesize\textsf{time}\ \\\ \\\ };
                \foreach \x in {1,...,7} {
                    \draw[bgLine] (\x,-0.2) --  (\x,0.2);
                \node at (\x, 0.5) {\normalsize{$\x$}};
            }
            \draw[axis] (1,0) -- (7.5,0);

            \foreach \middle/\level/\mdx/\color/\clock in {3.7/1/2/ca/\x_1, 4.2/2/2/cb/\x_2, 5/3/2/cc/\x_3} {

                \begin{pgfonlayer}{foreground}\node at (5-2.2, -\level/2) {$\mathsf{\clock}$};
                \end{pgfonlayer}

                \draw[line width=0.6mm,draw=white] (5,0.2) -- (5,-\level/2);
                \draw[line width=0.3mm] (\middle,0.2) -- (\middle,-\level/2);
                \draw[bgLine] (\middle,-0.2) --  (\middle,0.2);
                \node[fill=white,yshift=-0.4mm,inner sep=0] at (\middle, 0.5) {\underline{${\middle}$}};
                \foreach \dx in {-2,...,\mdx} {
                    \node[dot,opacity=0.5,inner sep=0.4mm] (dot) at (\middle+\dx,-\level/2) {};

                    \begin{pgfonlayer}{background}
                        \draw[dashed] (\middle+\dx,-\level/2) -- (\middle+\dx,0);
                    \end{pgfonlayer}

                    \node[line width=0.5mm,fill=accent, inner sep=0.7mm, outer sep=0, draw=white] at (\middle+\dx,0) {};
                }

                \begin{pgfonlayer}{background}
                    \draw [line width=1.6mm,draw=\color] (\middle-2.04,-\level/2) -- (\middle+2.04,-\level/2);
                \end{pgfonlayer}
                \node[dot] (dot) at (\middle,-\level/2) {};
            }

            \fill[fill=white, opacity=0.85] (5,-0.1) rectangle (7.2,-2);
            \fill[fill=white, opacity=0.85] (3,-0.1) rectangle (1,-2);
            \node[dot] (dot) at (5,-3/2) {};
            \draw[line width=0.6mm,draw=white] (5,-0.09) -- (5,-2);
            \draw[line width=0.3mm] (5,-0.09) -- (5,-2);
            \draw[line width=0.6mm,draw=white] (3,-0.09) -- (3,-2);
            \draw[line width=0.3mm] (3,-0.09) -- (3,-2);
            \node[fill=white,draw=black] (q) at (5, -2.1) {\scriptsize$\nowof{X}$};
            \draw[line width=0.3mm] (q.north west) -- (q.north east);
            \node[fill=white,draw=black] (q) at (3, -2.1) {\scriptsize$\nowof{X}-m$};
            \draw[line width=0.3mm] (q.north west) -- (q.north east);

        \end{tikzpicture}
%    \end{center}


==> membership.tex <==
% !TEX root = main.tex

\section{Membership problems}

In this section we establish the decidability status of \DTA and \kDTA{k} membership problems,
for \kNTA{1} languages.

\subsection{Decidability of \kDTA{k} membership for \kNTA{1}} % languages}

%In this section we prove the following result:

\begin{theorem} \label{thm:kDTA:memb}
For every fixed $k\geq 0$, the \kDTA{k} membership problem is decidable for \kNTA{1} languages.
\end{theorem}
%
\noindent
We build on the decision procedure of~\cite{OW04} which is easily adaptable to a slightly more general problem:
%
\begin{lemma}[\cite{OW04}] \label{lem:OW04}
It is decidable, for a given set of configurations $c_1, \dots, c_m$ of \NTA $A_1, \dots, A_m$, respectively, and
a given set of configurations $d_1, \dots, d_n$ of a \kNTA{1} $A$, whether
\[
\bigcup_{i\in\set{1,\dots, m}} \langtsa {A_i} {c_i} \quad \subseteq \quad 
\bigcup_{i\in\set{j,\dots, n}} \langtsa {A} {d_j}.
\]
\end{lemma}

Recall Fact~\ref{fact:supportagain}: for a timed word $w$ and a
\kDTA{k} $B$, the language $w^{-1} \langts B$ is \emph{$k$-supported},
by which we mean that it is supported by a set of cardinality
at most $(k+1)$ containing the last timestamp $t$ of $w$.
We use the following characterization (we embark on its proof later):
%
\begin{fact} \label{fact:memb-char-3}
	The following conditions are equivalent, for a \kNTA{1} $A$:
%	For an \NTAe $A$ and $k, m \geq 0$, 
	\begin{enumerate}
		\item $\langts A = \langts B$ for some \kDTA{k} $B$.	
		\item $w^{-1} \langts A$ is $k$-supported for each timed word $w$.
	\end{enumerate}
\end{fact}
%

\noindent
For proving \Cref{thm:kDTA:memb} we provide two semi-decision procedures:
%
\begin{itemize}
\item positive procedure: enumerate all \kDTA{k} $B$ and stop when $\langts A = \langts B$;
\item negative procedure: enumerate all timed words $w$ and stop when 
%
%\begin{align} \label{eq:tocheck}
$w^{-1} \langts A$ is \emph{not} $k$-supported.
%\end{align}
%
\end{itemize}

The equality test in the positive procedure reduces to checking two conditions:
disjointness of $\langts A$ and the complement $\overline{\langts B}$ (reducible to non-emptiness of the product automaton) and
the inclusion $\langts B \subseteq \langts A$ (decidable when $A$ is a \kNTA{1} by~\Cref{lem:OW04}).
Correctness of the negative procedure follows by Fact~\ref{fact:memb-char-3}.
We need to design a decision procedure to check, for a given timed word $w$, whether $w^{-1} \langts A$ is not $k$-supported.
For the sake of computability we restrict below our considerations, w.l.o.g., 
to timed words $w$ with \emph{rational} timestamps. 

Recall the timed transition system $\sem A$ consisting of discrete and time-elapse transitions. 
The time-elapse transitions are deterministic. 
The discrete transitions in $\sem A$ are non-deterministic,
but the branching is finite (and even bounded): the set $\succe a c = \setof{c'}{c \goesto{a} c'}$ is finite for every configuration $c$ and $a\in\Sigma$.

Let $t = t_n$ be the last timestamp in $w = (\startletter, t_0) (a_1, t_1) \dots (a_n, t_n)$.
%and $e = \delta_1 a_1 \dots \delta_n a_n = \es w$ be the elapse sequence determined by $w$.
By the above-discussed finite-branching of $\sem A$, the set
\[
\succe w c \ = \ \setof{c'}{c \goesto{t_1 - t_0} \goesto{a_1} \dots \goesto{t_n-t_{n-1}}\goesto{a_n} c'}
\]
is finite for every $c$, and hence so is also the set:
%
\begin{align} \label{eq:Xw}
X_w \ = \ \bigcup_{c \text{ initial}} \succe w c.
\end{align}
%
We observe the equality:
%
\begin{align} \label{eq:langunion}
w^{-1} \langts A \quad = \quad \bigcup_{c \in X_w} \langtsstarta A t {c}, % \quad =: \quad \langtsa A w
\end{align}
%
and thus we need to check if the  right-hand side language is $k$-supported.
As $A$ has just one clock and the timestamps in $w$ are rationals, 
configurations in $X_w$ are of the form $(p, \mu) \in \L \times \Qpos$.
Let $X_w = \set{(p_1, \mu_1), \dots, (p_l, \mu_l)}$.
%
As every $\langtsstarta A t {p_i, \mu_i}$ is supported by the set $\set{t - \mu_i, t}$, 
due to Fact~\ref{fact:support},
we have (put $L := \langts A$):
\begin{fact}
$w^{-1} L$ is $l$-supported, i.e., supported by the $(l+1)$-element set $S = \set{t - \mu_1, \dots, t - \mu_l, t}$.
\end{fact}
%
As only fractional parts of supporting timestamps matter (c.f.~Fact~\ref{fact:supp:int})
if $w^{-1} L$ is supported by a $(k+1)$-element set containing $t$, then it is also supported by such subset of $S$.
%w.l.o.g.~the subset contains $t$, as the last timestamp $t$ of $w$ is always necessary (up to fractional part) to support 
%any left quotient $w^{-1} L$.
We can thus check if $w^{-1} L$ is not $k$-supported by examining only subsets of $S$, as follows:
for every $k$-element subset $I \subseteq \set{1, \dots, l}$ (put $\mu'_i := \mu_i$ for $i \in I$), do the following:
%
\begin{enumerate}
%$T := \setof{t - \mu_i}{i\in I} \cup \set{t}$ and 
\item guess values $\mu'_i \in \Qpos$, for $i \in \set{1, \dots, l} - I$,  \st there is a timed automorphism $\pi$ satisfying
$\pi(t) = t$ and $\pi(t - \mu_i) = t - \mu'_i$ for $i\in I$;
\item check that %$w^{-1} L 
$\bigcup_{i\in\set{1, \ldots, l}} \langtsstarta A t {p_i, \mu_i} \ \neq \ \bigcup_{i\in\set{1, \ldots, l}} \langtsstarta A t {p_i, \mu'_i}$.
\end{enumerate}
%

\noindent
Indeed, the last point proves $w^{-1} L \ \neq \ \pi(w^{-1} L)$, and is decidable due to~\eqref{eq:t} and~\Cref{lem:OW04}.
%The first point amounts to guessing $\mu'_i$ up to the $k,m$-regions.

\begin{proof}[Proof of Fact~\ref{fact:memb-char-3}]
The implication $1 \Rightarrow 2$ follows by Fact~\ref{fact:supportagain}.
For the converse implication, $2 \Rightarrow 1$, consider an arbitrary fixed \kmNTA{1}{m} $A$ satisfying 2.
Put $L := \langts A$.
We are going to construct a \kDTA{k} $B$ such that $\langts B = L$.
%We apply \Cref{thm:DTA-char}. 
%Therefore, as $\langts A$ is necessarily $m$-forgetful by \Cref{lem:NTA:forgetful}, 
%it remains to show that
%it has only finitely many left quotients $w^{-1} \langts A$ up to timed automorphisms.

Fix a timed word $w$ with last timestamp $t$ and recall the set $X_w = \set{(p_1, \mu_1), \dots, (p_l, \mu_l)}$ as defined in~\eqref{eq:Xw}.
As the quotient $w^{-1} L$ is $k$-supported 
there is a subset $I_w \subseteq \set{1, \ldots, l}$ of cardinality at most $k$ \st
the set $T_w = \setof{t - \mu_i}{i\in I_w} \cup \set{t}$ supports $\langtsa A w$.
Denote by $\Pi_w$  be the set of all timed automorphisms that fix $T_w$; 
thus $w^{-1} L = \pi(w^{-1} L)$ for every $\pi \in \Pi_w$ 
and we deduce, using~\eqref{eq:langunion}, the following equalities:
%
\begin{align} 
\begin{aligned} \label{eq:sets}
w^{-1} L	    \ = \ & \ \ \bigcup_{\pi \in \Pi_w} \pi(w^{-1} L) \\
		    \ = \ & \ \ \bigcup_{\pi \in \Pi_w} \ \bigcup_{(p, \mu) \in X_w} \pi(\langtsstarta A {t} {p, \mu}) \\
		    \ = \ & \bigcup_{(p, \mu) \in X_w} \ \bigcup_{\pi \in \Pi_w}  \pi(\langtsstarta A {t} {p, \mu}). % \\
%		    \ = \ & \bigcup_{(p, \mu) \in X_w} \Pi_w(\langtsstarta A t {p, \mu}),
\end{aligned}
\end{align}
%
% where $\Pi_w(\langtsstarta A t {p, \mu}) := \bigcup_{\pi \in \Pi_w}  \pi(\langtsstarta A {t} {p, \mu})$.
Put $Y_w := \setof{(p_i, \mu_i)}{i\in I_w}$.
As automorphisms from $\Pi_w$ necessarily fix $\langtsstarta A t {p, \mu}$ for $(p, \mu) \in Y_w$,
%we have $\Pi_w(\langtsstarta A t {p, \mu}) = \langtsstarta A t {p, \mu}$,
\eqref{eq:sets} expands further to:
%
\begin{align*} 
\begin{aligned} 
% \langtsa A w   =  
			\bigcup_{(p, \mu) \in Y_w} \! \langtsstarta A t {p, \mu}  \ \ \cup \  
			\bigcup_{(p, \mu) \in X_w-Y_w} \ \bigcup_{\pi \in \Pi_w} \! \pi(\langtsstarta A t {p, \mu}).
\end{aligned}
\end{align*}
%



Assume, w.l.o.g., that $A$ is greedily-resetting; hence the numbers $\mu_i$ appearing in sets $X_w$
are bounded by $m$: $0 \leq \mu_i < m$ for $1\leq i \leq l$.
There are only finitely many possible $(k+1)$-tuples of reals of span bounded by $m$, up to timed automorphisms.
We formalize this intuition using the notion of \emph{orbit}: for a finite subset $S\subseteq \R$ and $\mu \in \R$, we define
the $S$-orbit of $\mu$ as
\[
\orb{S}{\mu} \ = \ \setof{\pi(\mu)}{\pi \text{ and automorphism fixing } S}.
\]

\islawek{to do}

Let $w$ range over all timed words.

This completes the proof of Fact~\ref{fact:memb-char-3}.
\end{proof}

\begin{remark}[Complexity]
	Both procedures invoke the \HyperAckermann-complete decision procedure of \Cref{lem:OW04}. %~\cite{OW04} .
	\HyperAckermann-hardness of the problem is stated in \Cref{cor:easy-undecidability}.
	We do not establish any complexity upper bound, % as we provide two separate semi-decision procedures only,
	but little effort is needed to turn the two partial procedures into one that always terminates and works in \HyperAckermann~time.
\end{remark}

\subsection{Lower bounds for \kDTA{k} membership problems}
\label{sec:easy-undecidability}

We show that, for every fixed $k \geq 0$,
the \kDTA{k} membership problem is undecidable for \kNTA{2} languages and for \kNTAe{1} languages.
We also prove \HyperAckermann-hardness of the \kDTA{k} membership problem for \kNTA{1} languages.
All the lower bounds are obtained by a reduction from the universality problem for the respective language 
classes (does a given language $L \subseteq \timedwords{\Sigma}$ satisfy $L = \timedwords{\Sigma}$?). The reduction is a suitable adaptation, generalization, and simplification
of an argument from \cite[Theorem 1]{Finkel:FORMATS:2006}
showing undecidability of \DTA membership for \NTA languages.

A timed language $L$ is \emph{timeless} if $L = \langts A$ for $A\in$ \kNTA{0} a timed automaton with no clocks
(hence timestamps appearing in input words are irrelevant for acceptance).
%
%We use below a non-standard operation of concatenation $\_ {\circ} \_$ of non-negative timed words $w, v$:
%\[
%w \circ v \quad := \quad w \cdot \, (t + v),
%\]
%where $t$ is the last time-stamp in $w$ ($t=0$ if $w = \varepsilon$), and
%the timed word $t + v$ is obtained by adding $t$ to all timestamps in $v$.
%The concatenation is lifted to non-negative timed languages in a standard way:
%\[
%L \circ K \quad := \quad \setof{w \circ v}{w \in L, v \in K}.
%\]
%and left quotient of a timed language $L$ with respect to a timed word $w$:
%\[
%w^{-1} L \quad := \quad \setof{v}{w \cdot v \in L}.
%\]


\begin{lemma} \label{lem:easy-undecidability}
	%
	Let $k \in \N$ and let $\mathcal Y$ be a class of timed languages that
	\begin{enumerate}
	\item contains all the timeless timed languages,
	\item is closed under union and concatenation: $K, L \in \mathcal {Y} \implies K\cup L, K\cdot L \in \mathcal Y$,  and
	\item contains some non-\kDTA{k} language.
	\end{enumerate}
	%
	The universality problem for languages in $\mathcal Y$ reduces in polynomial time
	to the \kDTA{k} membership problem for languages in $\mathcal Y$.
\end{lemma}

\begin{proof}
	 Consider some fixed timed language $M \in \mathcal Y$ which is not recognised by any \kDTA{k}
	(relying on the assumption 3), over an alphabet $\Gamma$.
	For a given timed language $L \in {\mathcal Y}$, over an alphabet $\Sigma$, we construct
	the following language over the extended alphabet $\Sigma \cup \Gamma \cup \{\$\}$ 
	with $\$ \not\in \Sigma \cup \Gamma$:
	%
	\begin{align*}
		N \; := \; L \cdot \{\$\} \cdot \timedwords{\Gamma} \;\cup\; \timedwords{\Sigma} \cdot \{\$\} \cdot M \ \subseteq \ \timedwords{\Sigma {\cup} \Gamma {\cup} \{\$\}},
		%\;\cup\; \setof{w \in \D^*} {\textrm{ $w$ contains $0$ or $\geq 2$ $\$$'s}}.
	\end{align*}
	where 
%	$\Gamma^*$ and $\Sigma^*$ stand for the timeless timed languages containing all timed words over $\Gamma$ and $\Sigma$, respectively, and 
	$\{\$\}$ stands for the timeless timed language over $\{\$\}$ consisting of all timed words of length 1.
	%
	Since $\mathcal Y$ contains all timeless timed languages due to the assumption 1, and is closed under
	union and concatenation due to the assumption 2, the language $N$ belongs to $\mathcal Y$.
	
	\begin{claim*}
		$L=\timedwords{\Sigma}$  if, and only if, $N$ is recognised by a \kDTA{k}.
	\end{claim*}

	For the ``only if'' direction, if $L = \timedwords{\Sigma}$ 
	then clearly $N = \timedwords{\Sigma} \cdot \{\$\} \cdot \timedwords{\Gamma}$.
	Thus  $N$ is timeless and in consequence $N$ is recognised by a \kDTA{k}, as \kDTA{k} recognise all timeless
	timed languages for any $k\geq 0$.
	
	For the ``if'' direction suppose, towards reaching a contradiction,
	that $N$ is recognised by a \kDTA{k} $A$
	but $L\neq\timedwords{\Sigma}$.
	Assume, w.l.o.g., that $A$ is greedily-resetting.
	Choose an arbitrary timed word $w = (\startletter, t_0) (a_1, t_1) \dots (a_n, t_n) \not\in L$ over $\Sigma$.
	Therefore, for any extension $v = (\startletter, t_0) (a_1, t_1) \dots (a_n, t_n) (\$, t_n + t)$ of $w$ by one letter, 
	we have
%	the left quotient $v^{-1}N$ equals $M$.
	\[  v^{-1} N = M. \] %\setof{u}{v \circ u \in N} \ = \ M. \]
	Choose $t$ larger than the largest absolute value $m$ of constants appearing in clock constraints in $A$, and
	let $(p, \mu)$ be the configuration reached by $A$ after reading $v$. 
	As $t > m$, all the clocks are reset by the last transition and hence $\mu(\x) = 0$ for all clocks $\x$.
	Consequently, if the initial control location of $A$ were moved to the location $p$, the so modified \kDTA{k} $A'$ would accept 
	the language $M$.
	But this contradicts our initial assumption that $M$ is not recognised by a \kDTA{k},
	thus finishing the proof.
\end{proof}


\begin{corollary}  \label{cor:easy-undecidability}
	%
	For every $k\geq 0$, the \kDTA{k} membership problem is:
	\begin{itemize}
	\item undecidable for \kNTA{2},
	\item undecidable for \kNTAe{1},
	\item \HyperAckermann-hard for \kNTA{1}.
	\end{itemize}
\end{corollary}

\begin{proof}
	All the three claims follow by~Lemma~\ref{lem:easy-undecidability}, which is applicable since
	each of the three classes contains all timeless timed languages, is closed under union and concatenation, and
	is not included in \kDTA{k} for any $k$
	(in particular, the \kNTA{1} language from Example~\ref{example:L1} is not recognised by any deterministic
	timed automaton).
	The universality problem is undecidable for \kNTA{2} as shown already in the seminal paper~\cite[Theorem 5.2]{AD94};
	quite similarly one shows undecidability for \kNTAe{1} \cite[Theorem 5.3]{LW0LasotaWalukiewicz:ATA:ACM088}.
	Finally, \HyperAckermann-hardness of the universality problem for \kNTA{1} follows form the
	same lower bound for the reachability problem in lossy channel systems~\cite[Theorem 5.5]{CS08},
	together with the reduction from this problem to universality of \kNTA{1} given in~\cite[Theorem 4.1]{LWLasotaWalukiewicz:ATA:ACM0808}.
\end{proof}

\subsection{Undecidability of \DTA membership for \kNTA{1}} % languages}

It has been shown in \cite[Theorem 1]{Finkel:FORMATS:2006} that it is undecidable
whether a \kNTA k timed language can be recognised by some \DTA, for any fixed $k \geq 2$.
%
The proof was a reduction from the \kNTA k universality problem,
which is undecidable for any fixed $k \geq 2$.
%
While the universality problem becomes decidable for $k = 1$,
we show in this section that the \DTA membership problem remains undecidable for \kNTA 1,
thus strengthening the result above.

\begin{theorem}
    The \DTA membership problem for \kNTA 1 languages is undecidable.
\end{theorem}

The idea is to reduce from the finiteness problem of lossy counter machines,
which is undecidable \cite[Theorem 13]{Mayr:TCS:2003}.
%
A \emph{$k$-counters lossy counter machine} (\kLCM k) is a tuple $M = \tuple {C, Q, q_0, \Delta}$,
where $C = \set{c_1, \dots, c_k}$ is a set of $k$ counters,
$Q$ is a finite set of control locations,
$q_0 \in Q$ is the initial control location,
and $\Delta$ is a finite set of instructions of the form $\tuple {p, \op, q}$,
where $\op$ is one of $\incr c$, $\decr c$, and $\ztest c$.
%
A configuration of an \LCM $M$ is a pair $\tuple {p, u}$,
where $p \in Q$ is a control location,
and $u \in \N^C$ is a counter valuation.
%
For two counter valuations $u, v \in \N^C$,
we write $u \leq v$ if $u(c) \leq v(c)$ for every counter $c \in C$.
%
The semantics of an \LCM $M$ is given by a (potentially infinite) transition system over the configurations of $M$
\st there is a transition $\tuple {p, u} \goesto \delta \tuple {q, v}$,
for
%either $\delta = \loss$, $p = q$, and $v \leq u$, or 
$\delta = \tuple {p, \op, q} \in \Delta$, whenever
%
%\begin{inparaenum}[1)]
\begin{enumerate}[1)]
    \item $\op = \incr c$ and $v \leq \extend c {u(c) + 1} u$, or
    \item $\op = \decr c$ and $v \leq \extend c {u(c) - 1} u$, or
    \item $\op = \ztest c$ and $u(c) = 0$ and $v \leq u$.
%\end{inparaenum}
\end{enumerate}
%
The \emph{finiteness problem} (a.k.a.~space boundedness) for an \LCM $M$
asks to decide whether the reachability set
$$\reachset M = \setof{\tuple{p, u}} {\tuple {q_0, u_0} \goesto {}^* \tuple{p, u}}$$
is finite, where $u_0$ is the constantly $0$ counter valuation.
%
\begin{theorem}[\protect{\cite[Theorem 13]{Mayr:TCS:2003}}]
    The \kLCM 4 finiteness problem is undecidable.
\end{theorem}

We use the following encoding of \LCM runs
as timed words over the alphabet $\Sigma = Q \cup \Delta \cup C$
(c.f.~\cite[Definition 4.6]{LasotaWalukiewicz:ATA:ACM08} for a similar encoding).
%
We interpret a counter valuation $u \in \N^C$
as the word over $\Sigma$
%
\begin{align*}
    u \;=\;
        \underbrace {c_1 c_1 \cdots c_1}_{u(c_1) \text{ letters}}\ 
            \underbrace {c_2 c_2 \cdots c_2}_{u(c_2) \text{ letters}}\ 
				\underbrace {c_3 c_3 \cdots c_3}_{u(c_3) \text{ letters}}\ 
					\underbrace {c_4 c_4 \cdots c_4}_{u(c_4) \text{ letters}}.
\end{align*}
%
With this interpretation, we encode an \LCM run
%
\begin{align*}
    \pi \;=\; \tuple{p_0, u_0}
        \goesto {\delta_1} \tuple{p_1, u_1}
            \goesto {\delta_2} \cdots
                \goesto {\delta_n} \tuple{p_n, u_n}
\end{align*}
%
as the timed word (backwards) called reversal-encoding of $\pi$,
%
\begin{align*}
    p_n \delta_n u_n\quad \cdots\quad p_1 \delta_1 u_1\quad p_0 u_0,
\end{align*}
%
\st $p_n$ occurs at time 0,
for every $1 \leq i < n$, $p_i$ occurs exactly after one time unit since $p_{i+1}$,
and if a ``unit'' of counter $c_1$ did not disappear due to lossiness when going from $u_i$ to $u_{i+1}$,
then the timestamps of the corresponding occurrences of letter $c_1$ in $u_i$ and $u_{i+1}$ are also at distance one
(and similarly for the other counters).
%
Under the encoding above, we can build a \kNTA 1 $A$ recognising the complement of the 
set of reversal-encodings of the runs of $M$.
The reversal operation is needed because $A$ does not have $\varepsilon$-transitions.
%
%
Intuitively, when reading a reversal-encoding of a run of $M$, % backwards,
the counters are allowed to spontaneously increase.
%
Therefore, the only kind of error that $A$ must verify is that some counter spontaneously decreases.
%
This can be done by guessing an occurrence of letter (say) $c_1$ in the current configuration
which does not have a corresponding occurrence in the next configuration after exactly one time unit.
%
This check can clearly be performed by an \NTA with one clock.
%
This reduction has the following property:
%
\begin{claim}
	The set of reachable configurations $\reachset M$ is finite
	if, and only if,
	$\lang A$ is a deterministic timed language.
\end{claim}

\begin{proof}
    For the ``only if'' direction, if $\reachset M$ is finite
    then there is some $k$ s.t.~every reachable configuration $u$ has size $u(c_1)+u(c_2)+u(c_3)+u(c_4)+1 \leq k$,
    and thus the set of reversals of accepting runs can be recognised by a \kDTA {(k+1)},
    and thus also its complement can be recognised by a $(k+1)$-\DTA.
    
    For the ``if'' direction, if $\reachset M$ is infinite,
    then there exist reachable configurations with arbitrarily large counter values.
    %
    Suppose, towards reaching contradiction, that $\lang A$ is recognised by a \kDTA k.
    Thus also its complement, that is the set of reversal-encodings of runs of $M$, is recognised by some \kDTA k $B$.
    %
    There exists a run $\pi$ of $M$ where some counter value exceeds $k$,
    and thus when $B$ reads the reversal-encoding of $\pi$ it must forget some timestamp (say) $\tuple {c_1, t}$
    in some configuration $p_{i+1} \delta_{i+1} u_{i+1}$.
    %
    Since $t$ is forgotten, we can perturb its corresponding $\tuple {c_1, t+1}$ in $p_i \delta_i u_i$
    to any value $\tuple {c_1, t'}$ \st $t' - t \neq 1$
    and obtain a new word still accepted by $A$,
    but which is no longer the reversal-encoding of a run of $M$,
    thus reaching the sought contradiction.
\end{proof}

\begin{remark}
	We observe that the reduction above uses a large alphabet $\Sigma$
	whose size depends on the input \LCM $M$.
	%
	In fact, an alternative encoding exists using a unary alphabet $\Sigma = \set{a}$.
	%
	Let the input \LCM $M$ have control locations $Q = \set{p_1, \dots, p_m}$
	and instructions $\Delta = \set{\delta_1, \dots, \delta_n}$.
	%
	An \LCM configuration $p_{j} \delta_{k} u$ is represented by the timed word consisting of 6 blocks
	%
	\begin{align*}
		\underbrace {a \cdots a}_{j \text{ letters}}
			\ \underbrace {a \cdots a}_{k \text{ letters}}
				\ \underbrace {a \cdots a}_{u(c_1) \text{ letters}}
					\ \underbrace {a \cdots a}_{u(c_2) \text{ letters}}
						\ \underbrace {a \cdots a}_{u(c_3) \text{ letters}}
							\ \underbrace {a \cdots a}_{u(c_4) \text{ letters}}
	\end{align*}
	%
	\st in each block the last $a$ is at timed distance exactly one from % the first $a$ of the same block.
	 the last $a$ of the previous block.
	%
	A unit of counter $c_1$ now repeats at distance $6$ in the next configuration (instead of $1$).
	%
	This shows that the \DTA membership problem is undecidable for
	\kNTA 1 using maximal constant $m=6$ over a unary alphabet.
\end{remark}
